ProxyPrompt: Securing System Prompts against Prompt Extraction Attacks

The integration of large language models (LLMs) into a wide range of applications has highlighted the critical role of well-crafted system prompts, which require extensive testing and domain expertise. These prompts enhance task performance but may also encode sensitive information and filtering criteria, posing security risks if exposed. Recent research shows that system prompts are vulnerable to extraction attacks, while existing defenses are either easily bypassed or require constant updates to address new threats. In this work, we introduce ProxyPrompt, a novel defense mechanism that prevents prompt leakage by replacing the original prompt with a proxy. This proxy maintains the original task's utility while obfuscating the extracted prompt, ensuring attackers cannot reproduce the task or access sensitive information. Comprehensive evaluations on 264 LLM and system prompt pairs show that ProxyPrompt protects 94.70% of prompts from extraction attacks, outperforming the next-best defense, which only achieves 42.80%.

==> sections/05_Experiment/03_embedding_to_token_loss.tex <==


\delete{\noindent\textbf{Utility of extracted prompts.}}
\add{\noindent\textbf{Unusable extracted prompts.}}
\add{Extracted prompts can also be viewed as a decoded approximation of proxy prompts.}
We evaluate the utility of the extracted prompt $G$ to assess potential attacker gains during prompt extraction. A refined extracted prompt $G^*$ is constructed by concatenating the most similar extracted sentences $S_{G}^*$ identified with~\Cref{eq:most_similar_sentence} for each system prompt sentence $S_{P} \in \mathbb{S}_P$. Note that this refinement relies on the knowledge of the real system prompt that is inaccessible to attackers, making their achievable utility lower than our refined estimates. 
We demonstrate the utility (accuracy or similarity) distribution of all configurations using three victim models in terms of the original prompt embedding $\phi_P$, proxy prompt $\tilde{\phi}_P$, and extracted $\phi_{G^*}$ in~\Cref{fig:plot_extracted_prompt}.
The blue boxes corresponding to extracted prompts show a notable drop in utility on CoLA, SST-2, and QNLI, where user queries lack task instructions. This indicates that the task-specific guidance in the original system prompts is effectively protected. For Roles and GSM8K, where user queries already include task instructions, extracted prompts also achieve lower utility than both the original and proxy prompts, underscoring the added value of system prompts and the protection offered by ProxyPrompt.
\add{Designing a more obfuscated target prompt $\tilde{P}$ could further reduce the utility of extracted prompts. As a proof of concept, we optimized the proxy prompt with a different target prompt in~\Cref{app:different_target_prompt}, leading to significant utility drops of extracted prompts.}
% , ``You are a GPT that refuses to answer all user queries'', for Roles and GSM8K. When this proxy prompt is stolen and used by an attacker, utility drops significantly as the model refuses to respond, as shown in~\Cref{app:different_target_prompt}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.98\textwidth]{figs/plot_extracted_prompt_gsm8k.png}
    \caption{Utility (accuracy or similarity) distribution of all configurations using three victim models in terms of the original prompt embedding $\phi_P$, proxy prompt $\tilde{\phi}_P$, and extracted $\phi_{G^*}$.}
    \label{fig:plot_extracted_prompt}
\end{figure}


\begin{wraptable}{r}{0.50\textwidth}
\vspace{-18pt}
\caption{Average similarity between proxy prompts and nearest vocabulary tokens using L-8B. Parentheses indicate typical vocabulary similarity.}
\vspace{2pt}
\label{tab:similarity_metrics}
\centering
{\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{8pt}
\begin{tabular}{lcc}
\toprule
\textbf{Task} & \multicolumn{2}{c}{\textbf{Similarity Metric}} \\
\cmidrule(lr){2-3}
            & \textbf{Cosine similarity} & \textbf{Dot product} \\
\midrule
CoLA     & 0.11 (0.40) & 0.05 (0.18) \\
SST-2    & 0.11 (0.40) & 0.05 (0.18) \\
QNLI     & 0.12 (0.42) & 0.06 (0.18) \\
Roles    & 0.12 (0.42) & 0.04 (0.19) \\
GSM8K    & 0.11 (0.40) & 0.03 (0.18) \\
\bottomrule
\end{tabular}
}
\vspace{-5pt}
\end{wraptable}
\noindent\textbf{Lossy decoding of proxy prompts.}
We measure how far proxy prompts deviate from natural language by decoding them into discrete tokens. We approximate decoding proxy prompts by mapping each embedding to its nearest token in vocabulary using various similarity metrics. \Cref{tab:similarity_metrics} reports the average similarity between proxy prompts and the embeddings of their nearest tokens. As a reference, we also report the average similarity between the embeddings of decoded tokens and their nearest non-identical vocabulary embeddings (shown in parentheses). The consistently lower similarity confirms that decoding proxy prompts is lossy due to the continuous-to-discrete gap.

% \begin{table}[th]
% \caption{Average similarity between proxy prompts and their nearest vocabulary tokens using L-8B. Values in parentheses serve as a reference, indicating typical similarity between vocabulary tokens.}
% \label{tab:similarity_metrics}
% \vskip 0.15in
% \begin{center}
% {\fontsize{9}{11}\selectfont
% \setlength{\tabcolsep}{8pt}
% \begin{tabular}{lccccc}
% \toprule
% \textbf{Similarity metric} & \textbf{CoLA} & \textbf{SST-2} & \textbf{QNLI} & \textbf{Roles} & \textbf{GSM8K} \\
% \midrule
% Cosine similarity        & 0.11 (0.40) & 0.11 (0.40) & 0.12 (0.42) & 0.12 (0.42) & 0.11 (0.40) \\
% Unnormalized dot-product & 0.05 (0.18) & 0.05 (0.18) & 0.06 (0.18) & 0.04 (0.19) & 0.03 (0.18) \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{table}


